Inference Latency Prediction at the Edge

With the growing workload of inference tasks on mobile devices, state-of-the-art neural architectures (NAs) are typically designed through Neural Architecture Search (NAS) to identify NAs with good tradeoffs between accuracy and efficiency (e.g., latency). Since measuring the latency of a huge set of candidate architectures during NAS is not scalable, approaches are needed for predicting end-to-end inference latency on mobile devices. Such predictions are challenging due to hardware heterogeneity, optimizations applied by ML frameworks, and the diversity of neural architectures. Motivated by these challenges, in this paper, we first quantitatively assess characteristics of neural architectures and mobile devices that have significant effects on inference latency. Based on this assessment, we propose a latency prediction framework which addresses these challenges by developing operation-wise latency predictors, under a variety of settings and a number of hardware devices, with multi-core CPUs and GPUs, achieving high accuracy in end-to-end latency prediction, as shown by our comprehensive evaluations. To illustrate that our approach does not require expensive data collection, we also show that accurate predictions can be achieved on real-world NAs using only small amounts of profiling data.

==> content/acknowledgment.tex <==

\section*{Acknowledgment}


==> content/result_0729.tex <==

\section{Results} \label{sec:result}

In this section, we evaluate our predicting framework with various ML approaches on two tasks: 
(1) Training data and test data are both from the synthetic dataset (\cref{sec:task_same_distribution}), and (2) the training data are from the synthetic dataset while the test data are the 102 real-world neural architectures (\cref{sec:task_different_distribution}). For each task, we first compare the predictions of different ML approaches on mobile CPUs with a large core and mobile GPUs, using floating point representations; then we thoroughly evaluate the best approach across all scenarios, including various combinations of cores and integer representations after quantization.


\subsection{Task I: Predictions on Neural Architectures from Same Distribution}\label{sec:task_same_distribution}

In the first task, we consider a common situation of NAS: 
To efficiently evaluate the efficiency metrics (e.g., latency) of each candidate neural architecture during NAS, a small number of neural architectures in the search space are profiled on each target device in advance, in order to build a prediction model which can accurately predict the latency of unseen neural architectures.
%
We assume that the training data are a set of neural architectures uniformly sampled from the search space, and the test data are the candidate neural architectures searched by NAS, which, for simplicity, are also considered as uniformly distributed over the search space.
%
Particularly, we randomly sample 100 neural architectures from the synthetic dataset as the test data, and use 30, 100 or 900 neural architectures from the rest of synthetic dataset as the training data to study the effects of training size.


\subsubsection{Comparison of ML Models}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_cpu_conv.pdf}
		\caption{Convolution}\label{fig:comparison_nas_cpu_conv}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_cpu_depthwise.pdf}
		\caption{Depthwise}\label{fig:comparison_nas_cpu_depthwise}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_cpu_end_to_end.pdf}
		\caption{End-to-end}\label{fig:comparison_nas_cpu_end_to_end}
	\end{subfigure}
	\caption{Predictions of ML Models on CPUs with a Large Core (Synthetic Neural Architectures in Floating Point)}
	\label{fig:comparison_nas_cpu}
\end{figure}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_gpu_conv.pdf}
		\caption{Convolution}\label{fig:comparison_nas_gpu_conv}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_gpu_depthwise.pdf}
		\caption{Depthwise}\label{fig:comparison_nas_gpu_depthwise}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_gpu_fc.pdf}
		\caption{FC}\label{fig:comparison_nas_gpu_fc}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_nas_gpu_end_to_end.pdf}
		\caption{End-to-end}\label{fig:comparison_nas_gpu_end_to_end}
	\end{subfigure}
	\caption{Predictions of ML Models on GPUs (Synthetic Neural Architectures in Floating Point)}
	\label{fig:comparison_nas_gpu}
\end{figure}

\paragraph{Mobile CPUs} \cref{fig:latency_breakdown_nas_cpu} reveals that convolution and depthwise convolution operations typically account for over 90\% end-to-end latency on mobile CPUs for the synthetic neural architectures.
%
Accordingly, \cref{fig:comparison_nas_cpu_conv,fig:comparison_nas_cpu_depthwise} compare the predictions from multiple ML approaches on both operations by displaying the average MAPE over four platforms;
%
as can be seen, the predictions of simple linear model (i.e., Lasso) are less sensitive to the size of training data, while all the sophisticated approaches achieve substantial improvements when training size increased from 30 to 900.
%
With sufficient training data (e.g., 900 neural architectures), all the sophisticated approaches acquire accurate predictions: For convolution operations, RF, GBDT and MLP achieve comparable predictions with 2.6\%, 2.5\% and 2.6\% errors respectively. At the same time, since GBDT outperforms other approaches on depthwise operations with 3.7\% error, the approach with best end-to-end predictions on mobile CPUs is GBDT, with only 2.4\% error shown in \cref{fig:comparison_nas_cpu_end_to_end}.


\paragraph{Mobile GPUs} As shown in \cref{fig:latency_breakdown_nas_gpu}, convolution, depthwise convolution, and fully-connected are the top three contributors to the end-to-end latency of synthetic neural architectures on mobile GPUs.
%
\cref{fig:comparison_nas_gpu} shows that with 900 training size, GBDT obtain the best predictions on both convolution (5.8\% error) and depthwise convolution (4.2\% error), as well as the end-to-end latency (6.3\% errors).

Overall, with sufficient training data, GBDT achieves best predictions on the 100 synthetic neural architectures. As a representative of sophisticated approaches, in the following section, we comprehensively evaluate the predictions from GBDT across various scenarios, using 900 synthetic neural architectures as the training data.


\subsubsection{Evaluation on GBDT with Training Size 900}
\paragraph{Mobile CPUs}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_s10_conv_mape.pdf}
		\caption{Exynos 9820}\label{fig:nas_cpu_s10_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_pixel4_conv_mape.pdf}
		\caption{Snapdragon 855}\label{fig:nas_cpu_pixel4_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_a03s_conv_mape.pdf}
		\caption{Helio P35}\label{fig:nas_cpu_a03s_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_mi8se_conv_mape.pdf}
		\caption{Snapdragon 710}\label{fig:nas_cpu_mi8se_conv_mape}
	\end{subfigure}
	\caption{Predictions of GBDT on Convolution with Multiple CPU Cores (Synthetic Neural Architectures)}
	\label{fig:nas_cpu_conv_mape}
\end{figure}


\cref{fig:nas_cpu_conv_mape} presents the predictions of GBDT on convolution operations, across various combinations of CPU cores, with both floating point and integer representations. 
%
As can be seen, an increasing number of homogeneous cores typically leads to higher prediction errors. Utilizing more cores can result in larger system variance, due to competing resources with the background jobs running on mobile devices (e.g., camera, sensors, and networking services); the system variance can impair the quality of profiling results and thus affect the prediction accuracy.
%
For example, from the results of Snapdragon 710 shown in \cref{fig:nas_cpu_mi8se_conv_mape}, the error of 6 small cores is significantly higher than of 1 small core for both data representations, due to the substantial interference from background jobs when an inference task attempts to make use of all the efficient cores on the device.
%
The combination of heterogeneous cores also shows a high prediction error, mainly accounted for the high variance from paralleling the execution of each operation with cores from different clusters, since inter-cluster communication cost is particularly higher than intra-cluster \cite{wang2019high}.


\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_s10_end_to_end_mape.pdf}
		\caption{Exynos 9820}\label{fig:nas_cpu_s10_end_to_end_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_pixel4_end_to_end_mape.pdf}
		\caption{Snapdragon 855}\label{fig:nas_cpu_pixel4_end_to_end_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_a03s_end_to_end_mape.pdf}
		\caption{Helio P35}\label{fig:nas_cpu_a03s_end_to_end_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_cpu_mi8se_end_to_end_mape.pdf}
		\caption{Snapdragon 710}\label{fig:nas_cpu_mi8se_end_to_end_mape}
	\end{subfigure}
	\caption{Predictions of GBDT on End-to-end Latency with Multiple CPU Cores (Synthetic Neural Architectures)}
	\label{fig:nas_cpu_end_to_end_mape}
\end{figure}


\cref{fig:nas_cpu_end_to_end_mape} displays the predictions on CPU end-to-end latency with GBDT, which is dominated by the error of convolution operations, which takes over 80\% of the end-to-end latency.
%
Another reason of the higher prediction errors of end-to-end latency for heterogeneous cores is that, some operations lacking the support of multithreading implementation can be scheduled on arbitrary core and thus show distinct performance over time, which also causes high variance in the measurements. 
%
As can be seen, GBDT achieves accurate predictions across all platforms: the worse cases for homogeneous cores are 13.17\% for Exynos 9820, 5.29\% for Snapdragon 855, 3.96\% on Helio P35, and 7.31\% for Snapdragon 710.


\paragraph{Mobile GPUs}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_gpu_conv_mape.pdf}
		\caption{Convolution}\label{fig:nas_gpu_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_gpu_depthwise_mape.pdf}
		\caption{Depthwise}\label{fig:nas_gpu_depthwise_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_gpu_fc_mape.pdf}
		\caption{FC}\label{fig:nas_gpu_fc_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/nas_gpu_end_to_end_mape.pdf}
		\caption{End-to-end}\label{fig:nas_gpu_end_to_end_mape}
	\end{subfigure}
	\caption{Predictions of GBDT on GPUs (Synthetic Neural Architectures in Floating Point)}
	\label{fig:nas_gpu_mape}
\end{figure}

\cref{fig:nas_gpu_mape} presents the predictions of GBDT across different GPUs, including three important operations which take a large proportion of the end-to-end latency.
%
For convolution operations, we split the results on Conv2D and Winograd kernels in \cref{fig:nas_gpu_conv_mape} since separate predictors are built for each kernel; there is no Winograd kernel generated for Adreno 640 and 616 due to the hardware dependency of the kernel selection algorithm as introduced in \cref{sec:kernel_selection}.
%
For Mali G76, the end-to-end latency predictions (6.4\%) are substantially higher than Conv2D kernels (4.5\%), due to the worse predictions on other kernels (Winograd, depthwise and fully-connected).
%
Overall, GBDT achieves promising end-to-end predictions on all four mainstream GPUs, with the maximum error 8.2\%.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Task II: Predictions on Neural Architectures from Different Distribution}\label{sec:task_different_distribution}

Next, we evaluate on another task in which the training data represent a small number of neural architectures sampled at the early stage of NAS, while the test data are the representative neural architectures (i.e., with promising accuracy) at the end of NAS. It turns out that the distributions between training data and test data are not necessarily consistent.
%
In our evaluation, we simulate the situation by using 102 real-world neural architectures as the test data, and 30, 100 or 1000 synthetic neural architectures as the training data to study effects of training size. 
%
The two sets of neural architectures are differently distributed; particularly, we observe that the latency of convolution operations in real-world neural architectures are overall smaller than these in the synthetic neural architectures.


\subsubsection{Comparison of ML Models}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_cpu_conv.pdf}
		\caption{Convolution}\label{fig:comparison_common_cpu_conv}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_cpu_depthwise.pdf}
		\caption{Depthwise}\label{fig:comparison_common_cpu_depthwise}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_cpu_end_to_end.pdf}
		\caption{End-to-end}\label{fig:comparison_common_cpu_end_to_end}
	\end{subfigure}
	\caption{Overall Predictions of ML Models on CPUs with a Large Core (Real-world Neural Architectures in Floating Point)}
	\label{fig:comparison_common_cpu}
\end{figure}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_gpu_conv.pdf}
		\caption{Convolution}\label{fig:comparison_common_gpu_conv}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_gpu_depthwise.pdf}
		\caption{Depthwise}\label{fig:comparison_common_gpu_depthwise}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_gpu_fc.pdf}
		\caption{FC}\label{fig:comparison_common_gpu_fc}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/comparison_common_gpu_end_to_end.pdf}
		\caption{End-to-end}\label{fig:comparison_common_gpu_end_to_end}
	\end{subfigure}
	\caption{Overall Predictions of ML Models on GPUs (Real-world Neural Architectures in Floating Point)}
	\label{fig:comparison_common_gpu}
\end{figure}


\paragraph{Mobile CPUs} \cref{fig:comparison_common_cpu} shows the predictions for the real-world neural architectures on CPUs.
%
Similarly to our observation in the previous task, adding more training data can improve the operation-wise predictions of all approaches. 
%
Besides, the end-to-end latency predictions largely depend on convolution; the only exception is MLP, which shows a huge error for other operations (e.g., the errors on Pooling operations are 585.45\%, 1281.23\% and 948.15\% on Pixel 4 with training sizes of 30, 100 and 1000 respectively) and thus the end-to-end latency predictions are significantly worse than convolution operations.


For most ML approaches trained on synthetic neural architectures, the prediction errors on the real-world neural architectures are higher than the results of synthetic neural architectures (in \cref{fig:comparison_nas_cpu}) which are generated from the same distribution as the training data.
%
The only exception is Lasso, which exhibits a better performance on the real-world neural architectures.
%
In fact, across all sizes of training data evaluated in this task, Lasso achieves the best predictions for both operations, as well as the end-to-end latency. 
%
We believe the reason is that, due to the loss function defined as MAPE, the prediction model are trained toward the direction which favors the fast operations with small latency than the ones with large latency. With less freedom than other sophisticated ML approaches, the linear model in Lasso can only fit well to the fast operations, resulting in higher accuracy for the real-world neural architectures of which the fast operations take a large proportion of the end-to-end latency.
%
% while other machine learning models can better fit into the synthetic neural architectures with same distribution as the training data, the linear model learned by Lasso generalizes better to unseen configurations of operations.

Another advantage of Lasso is the small amount of training data (e.g., 30 neural architectures) required to obtain accurate predictions. As can be seen, the results of Lasso are less sensitive to the size of training dataset than other ML approaches; specifically, Lasso outperforms other approaches with 6.9\%, 6.3\% and 5.7\% errors when trained on 30, 100, and 1000 synthetic neural architectures respectively.
%
As pointed out by prior work \cite{lu2021one}, the cost of profiling only 30 neural architectures on each target device is negligible compared to the time-consuming process of NAS.



\paragraph{Mobile GPUs}
\cref{fig:comparison_common_gpu} presents the predictions on mobile GPUs.
%
We observe that, for some small real-world neural architectures, the overhead of running inference kernel-independent code (as shown in \cref{fig:gpu_overhead}) can significantly affect the end-to-end latency. Since the overhead sometimes vary in a large range (e.g., for PowerVR GE8320 and Mali G76), it can largely affect the end-to-end latency prediction.
%
With sufficient training data of 1000 neural architectures, Lasso achieves slightly worse end-to-end latency predictions (8.8\%) than RF (7.6\%) and GBDT (7.6\%); in the case of scarce training data with only 30 neural architectures, Lasso achieves the best end-to-end latency predictions (9.1\%).

Overall, Lasso achieves the best predictions for the real-world neural architectures. In the following section, we comprehensively evaluate the results from Lasso across different scenarios, using 30 synthetic neural architectures as the training data.

\subsubsection{Evaluation on Lasso with Training Size 30}

\paragraph{Mobile CPUs} 

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_s10_conv_mape.pdf}
		\caption{Exynos 9820}\label{fig:common_cpu_s10_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_pixel4_conv_mape.pdf}
		\caption{Snapdragon 855}\label{fig:common_cpu_pixel4_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_a03s_conv_mape.pdf}
		\caption{Helio P35}\label{fig:common_cpu_a03s_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_mi8se_conv_mape.pdf}
		\caption{Snapdragon 710}\label{fig:common_cpu_mi8se_conv_mape}
	\end{subfigure}
	\caption{Predictions of Lasso on Convolution with Multiple CPU Cores (Real-world Neural Architectures)}
	\label{fig:common_cpu_conv_mape}
\end{figure}

\cref{fig:common_cpu_conv_mape} displays the predictions of Lasso across various combinations of cores and data representations; generally, the trend of prediction errors for homogeneous and heterogeneous clusters are similar to the previous results, as higher system variance impair the prediction accuracy.

Since all the features are already standardized in \cref{eq:standardization}, we use the magnitude of weights in the Lasso model to analyze the importance of different features. On all platforms, we find the most critical feature of convolution operation is FLOPs, which still considerably reflect the computational complexity of a neural architecture, even if not an accurate proxy metric for the actual latency. In addition, we observe that the second largest weight across all devices is always assigned to the kernel size, which represents the number of parameters for the convolution and reflects the cost of memory access.


\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_s10_end_to_end_mape.pdf}
		\caption{Exynos 9820}\label{fig:common_cpu_s10_end_to_end_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_pixel4_end_to_end_mape.pdf}
		\caption{Snapdragon 855}\label{fig:common_cpu_pixel4_end_to_end_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_a03s_end_to_end_mape.pdf}
		\caption{Helio P35}\label{fig:common_cpu_a03s_end_to_end_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_cpu_mi8se_end_to_end_mape.pdf}
		\caption{Snapdragon 710}\label{fig:common_cpu_mi8se_end_to_end_mape}
	\end{subfigure}
	\caption{Predictions of Lasso on End-to-end Latency with Multiple CPU Cores (Real-world Neural Architectures)}
	\label{fig:common_cpu_end_to_end_mape}
\end{figure}

\cref{fig:common_cpu_end_to_end_mape} presents the end-to-end latency predictions of Lasso on the real-world neural architectures.
%
The maximum errors for combinations of homogeneous cores are 22.9\% on Exynos 9820, 13.5\% on Snapdragon 855, 9.6\% on Helio P35, and 10.9\% on Snapdragon 710. We believe the large prediction errors on Exynos 9820 is attributed to the large system variance from occupying many small efficient cores, which can affect the quality of training data and severely impair the predictions in the case of scarce training data. As can be seen, the prediction errors can be improved to less than 14.8\% when adding more training data.

Across all devices, the worst case typically appears in the case of utilizing all small cores, due to the interference from the background jobs scheduled on the cluster of efficient cores. One exception is Helio P35, where the predictions on large and small cores show similar errors; we believe that the reason is related to the similarity between the two core clusters on Helio P35, since both core clusters are Cortex-A53 but runing in different clock speeds (as shown in \cref{table:feature}). 

\paragraph{Mobile GPUs} 

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_gpu_conv_mape.pdf}
		\caption{Convolution}\label{fig:common_gpu_conv_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_gpu_depthwise_mape.pdf}
		\caption{Depthwise}\label{fig:common_gpu_depthwise_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_gpu_fc_mape.pdf}
		\caption{FC}\label{fig:common_gpu_fc_mape}
	\end{subfigure}
	\begin{subfigure}[b]{.245\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/results/common_30_gpu_end_to_end_mape.pdf}
		\caption{End-to-end}\label{fig:common_gpu_end_to_end_mape}
	\end{subfigure}
	\caption{Predictions of Lasso on GPUs (Real-world Neural Architectures in Floating Point)}
	\label{fig:common_gpu_mape}
\end{figure}

\cref{fig:common_gpu_conv_mape,fig:common_gpu_depthwise_mape,fig:common_gpu_fc_mape} show the operation-wise latency predictions of Lasso across various mobile GPUs.
%
For convolution kernels on mobile GPUs, FLOPs and kernel size are still the two most important features with substantial weights in the Lasso model, which is consistent with the results on mobile CPUs.
%
Different from convolution kernels, the top two critical features of depthwise kernels are FLOPs and input size.
%
Because the depthwise convolution is applied to each channel separately, the parameter size of depthwise convolution is substantially smaller than standard convolution.
%
As a result, the size of the input tensor dominates the cost of memory access for depthwise convolution.

\cref{fig:common_gpu_end_to_end_mape} shows the end-to-end latency predictions of Lasso on mobile GPUs. 
%
In general, the predictions on the slower GPUs (5.0\% on PowerVR GE830 and 5.4\% on Adreno 616) are better than the faster GPUs (11.0\% on Mali G76 and 10.7\% on Adreno 640), as we observe smaller variance on the slower GPUs over the longer execution time.


% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}[b]{.4\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figures/performance_box_plot/effect_kernel_selection_winograd_s10_outliers.pdf}
% 		\caption{Exynos 9820 (Mali G76)}\label{fig:effect_kernel_selection_winograd_s10}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{.4\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figures/performance_box_plot/effect_kernel_selection_winograd_a03s_outliers.pdf}
% 		\caption{Helio P35 (PowerVR GE8320)}\label{fig:effect_kernel_selection_winograd_a03s}
% 	\end{subfigure}
% 	\caption{Predictions on Winograd Kernels}
% 	\label{fig:effect_kernel_selection_winograd}
% \end{figure}

% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}[b]{.4\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figures/performance_box_plot/effect_kernel_selection_end-to-end_s10_outliers.pdf}
% 		\caption{Exynos 9820 (Mali G76)}\label{fig:effect_kernel_selection_end-to-end_s10_outliers}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{.4\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{figures/performance_box_plot/effect_kernel_selection_end-to-end_a03s_outliers.pdf}
% 		\caption{Helio P35 (PowerVR GE8320)}\label{fig:effect_kernel_selection_end-to-end_a03s}
% 	\end{subfigure}
% 	\caption{Predictions on End-to-End Latency for Models with Winograd kernels}
% 	\label{fig:effect_kernel_selection_end-to-end}
% \end{figure}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.4\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/performance_box_plot/effect_kernel_selection_winograd_a03s_outliers.pdf}
		\caption{Winograd Kernel Latency}\label{fig:effect_kernel_selection_winograd_a03s}
	\end{subfigure}
	\begin{subfigure}[b]{.4\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/performance_box_plot/effect_kernel_selection_end-to-end_a03s_outliers.pdf}
		\caption{End-to-end Latency}\label{fig:effect_kernel_selection_end-to-end_a03s}
	\end{subfigure}
	\caption{Predictions on Helio P35 (PowerVR GE8320) for Whether Distinguishing Winograd Kernels}
	\label{fig:effect_kernel_selection_a03s}
\end{figure}
